See2Refine: Vision-Language Feedback Improves LLM-Based eHMI Action Designers

Automated vehicles lack natural communication channels with other road users, making external Human-Machine Interfaces (eHMIs) essential for conveying intent and maintaining trust in shared environments. However, most eHMI studies rely on developer-crafted message-action pairs, which are difficult to adapt to diverse and dynamic traffic contexts. A promising alternative is to use Large Language Models (LLMs) as action designers that generate context-conditioned eHMI actions, yet such designers lack perceptual verification and typically depend on fixed prompts or costly human-annotated feedback for improvement. We present See2Refine, a human-free, closed-loop framework that uses vision-language model (VLM) perceptual evaluation as automated visual feedback to improve an LLM-based eHMI action designer. Given a driving context and a candidate eHMI action, the VLM evaluates the perceived appropriateness of the action, and this feedback is used to iteratively revise the designer's outputs, enabling systematic refinement without human supervision. We evaluate our framework across three eHMI modalities (lightbar, eyes, and arm) and multiple LLM model sizes. Across settings, our framework consistently outperforms prompt-only LLM designers and manually specified baselines in both VLM-based metrics and human-subject evaluations. Results further indicate that the improvements generalize across modalities and that VLM evaluations are well aligned with human preferences, supporting the robustness and effectiveness of See2Refine for scalable action design.

==> sections/6_discuss.tex <==
\section{Discussion}
\textbf{Human-augmented co-learning.} A natural extension is to let a small amount of human judgment anchor the evaluator used in our loop. Instead of collecting labels for every generated eHMI action, human raters can focus on cases where automatic scores are most uncertain or where social interpretation matters most (e.g., ambiguous right-of-way, low-visibility scenes, culturally sensitive wording). These human scores can be distilled into a light human preference model (HPM) and then combined with the VLM to form a mixed evaluator. The VLM keeps coverage and speed, while the HPM injects human semantics and social priors. This allows us to scale human intent to a large synthetic pool without linearly scaling human effort.

\textbf{Efficiency-oriented iteration.} The current loop can be made faster by changing how samples are admitted to the expensive stages. One route is difficulty- or uncertainty-based scheduling: only actions whose VLM and HPM disagree, or actions for complex scenes, go through full evaluation and preference optimization; actions for simple, high-confidence scenes are evaluated once. A second route is staged evaluation: a light model (small VLM or the HPM) does fast filtering, and only top candidates are passed to the full evaluator. A third route is asset reuse: if the same scene and viewpoint are rendered once, later eHMI variants reuse the render instead of re-generating it. Together, these tactics reduce wall-clock time per round and make more co-learning iterations feasible under the same compute budget.

\textbf{Improving evaluator reliability.} Even with a mixed evaluator, score drift can appear over long training runs. Periodically refreshing the HPM with a small new batch of human ratings, especially on failure patterns discovered by the VLM, can keep the evaluation space stable. Another option is to log evaluator disagreements and replay them as hard negatives during preference optimization. Both strategies keep the designer model aligned with human-facing judgments without requiring continuous human annotation.

\section{Conclusion}
We showed that an LLM–VLM co-learning pipeline can refine eHMI actions without large human-labeled datasets. To make the method practical at scale, future work should (i) insert targeted human feedback and distill it into an HPM to guide automatic evaluators, (ii) restructure the loop with uncertainty-based scheduling, staged evaluation, and render reuse to lower iteration cost, and (iii) periodically refresh evaluator signals to prevent drift. These steps keep the system efficient while moving its behavior closer to human traffic communication.

